Random Permutation Codes: Lossless Source Coding of Non-Sequential Data

This thesis deals with the problem of communicating and storing non-sequential data. We investigate this problem through the lens of lossless source coding, also sometimes referred to as lossless compression, from both an algorithmic and information-theoretic perspective. Lossless compression algorithms typically preserve the ordering in which data points are compressed. However, there are data types where order is not meaningful, such as collections of files, rows in a database, nodes in a graph, and, notably, datasets in machine learning applications. Compressing with traditional algorithms is possible if we pick an order for the elements and communicate the corresponding ordered sequence. However, unless the order information is somehow removed during the encoding process, this procedure will be sub-optimal, because the order contains information and therefore more bits are used to represent the source than are truly necessary. In this work we give a formal definition for non-sequential objects as random sets of equivalent sequences, which we refer to as Combinatorial Random Variables (CRVs). The definition of equivalence, formalized as an equivalence relation, establishes the non-sequential data type represented by the CRV. The achievable rates of CRVs is fully characterized as a function of the equivalence relation as well as the data distribution. The optimal rates of CRVs are achieved within the family of Random Permutation Codes (RPCs) developed in later chapters. RPCs randomly select one-of-many possible sequences that can represent the instance of the CRV. Specialized RPCs are given for the case of multisets, graphs, and partitions/clusterings, providing new algorithms for compression of databases, social networks, and web data in the JSON file format.

==> texts/future.tex <==
\chapter{Future Work}

==> texts/nonsense/nonsense-ans.tex <==
For this savings to be realized, the initial state must be above a minimum threshold that is a function of the information content of $Z_1$.
\begin{example}[Initial Bits]
    Let $X_1 = x_1$ be the first observation to be encoded in the BB-ANS procedure.
    Assume $- \log Q_{Z \g X}(z \g x_1) = 10$ bits, a quantized uniform distribution on $\abs{\Z} = 2^{10}$ elements, with precision $N_Z=2^{10}$, for all $z$.
    If $\log s_0 = 32$ bits,
    \begin{align}
        s_0^\prime, z_1 = \decode(s_0, Q_{Z \g X}(\cdot \g x_1)),
    \end{align}
    gives,
    \begin{align}
        z_1 = s_0 \bmod N_Z =  2^{32} \bmod 2^{10} = 0
    \end{align}
    implying $c_z = 0$, assuming $0$ is the fist symbol in the alphabet, $p_z = 1$, and,
    \begin{align}
        \log s_0^\prime & = \log \left(p_z \cdot (s_0 \div N_Z) + s_0 \bmod N_Z - c_z\right) \\
                        & = \log \left(1 \cdot (2^{32} \div 2^{10}) + 0 - 0 \right)          \\
                        & = 22 \text{ bits}.
    \end{align}
    This totals a savings of exactly the information content of the latent, $\log(s_0) - \log(s_0^\prime) = 10$ bits.
    However, consider the initial state $\log s_0 = 8$.
    This state is smaller than $10$ bits and decodes to,
    \begin{align}
        z_1 = s_0 \bmod N_z = 2^8 \bmod 2^{10} = 2^8.
    \end{align}
    Since the distribution is uniform and the number of elements is equal to the precision, $\abs{\Z} = N_Z$, then we have that $c_z = z$ for all values of $z$.
    After decoding the new state equals $0$,
    \begin{align}
         & p_z \cdot (s_0 \div N_Z) + s_0 \bmod N_Z - c_z        \\
         & = 1\cdot (2^8 \div 2^{10}) + (2^8 \bmod 2^{10}) - 2^8 \\
         & = 0,                                                  \\
    \end{align}
    which equals a reduction in the state less than the information content
\end{example}
The previous example highlights the issue with letting the initial state reach $0$ during the sampling step.
The next state was $0$ when decoding from either $2^7$ and $2^8$, and hence the decoder, upon receiving a state at $0$, would not be able to restore the state to its correct value before encoding, due to this ambiguity.
We can show the initial bits problem occurs when the initial state is equal to one of the cumulative quantized likelihood values, $s_0 = c_z$, for some $z \in \Z$.
\begin{theorem}
    Let $p_z, c_z$ be the quantized likelihood and cumulative likelihood values of some quantized probability distribution over an alphabet $\Z$.
    Then, if the initial state is equal to one of the cumulative quantized probability values,
    \begin{align}
        s_0 \in \{c_z \colon z \in \Z\},
    \end{align}
    sampling with ANS will result in the initial bits problem.
\end{theorem}
\begin{proof}
    To avoid the initial bits problem, the initial state $s_0$ must satisfy,
    \begin{align}\label{eq:initial-bits-cond}
        p_z \cdot (s_0 \div N_Z) + s_0 \bmod N_Z - c_z > 0,
    \end{align}
    for all $z \in \Z$. Since $z$ is the decoded symbol: $s_0 \bmod N_Z \in [c_z, c_z + p_z)$, implying $s_0 \bmod N_Z \geq c_z$.

    If $s_0 \geq N_Z$, then $p_z \cdot (s_0 \div N_Z) \geq p_z > 0$.
    This gives,
    \begin{align}
         & p_z \cdot (s_0 \div N_Z) + s_0 \bmod N_Z - c_z &  &                          \\
         & \geq p_z \cdot (s_0 \div N_Z)                  &  & (s_0 \bmod N_Z \geq c_z) \\
         & \geq p_z                                       &  & (s_0 \geq N_Z)           \\
         & > 0.
    \end{align}
    For $s_0 < N_Z$,
    \begin{align}
         & p_z \cdot (s_0 \div N_Z) + s_0 \bmod N_Z - c_z &  &                       \\
         & = s_0 \bmod N_Z - c_z                          &  & (s_0 \div N_Z = 0)    \\
         & = s_0 - c_z                                    &  & (s_0 \bmod N_Z = s_0) \\
         & \geq 0.
    \end{align}
    The value of $c_z$ depends on which range the initial state is in, $s_0 \in [c_z, c_z + p_z)$, which also defines the decoded symbol $z$.
    However, for any decoded $z$, it is true that $c_z \leq s_0$, with the initial bits problem occurring only at equality.
\end{proof}
ANS defines codes of sequences of observations by encoding symbols sequentially into a common ANS state.
The first step of encoding is always to sample a latent with an ANS decode.
This means the depletion of the ANS state is not restricted to the sampling of $Z_1$, but can happen for any $Z_i$.

It is therefore sufficient, but not necessary, to set $s_0 \geq N_Z$ to avoid the initial bits issue, as $c_z < N_Z$ for all latent values.
